Adapting LLM Agents with Universal Feedback in Communication

Recent advances in large language models (LLMs) have demonstrated potential for LLM agents. To facilitate the training for these agents with both linguistic feedback and non-linguistic reward signals, we introduce Learning through Communication (LTC). We design a universal buffer to store all the feedback, and an iterative pipeline to enable an LLM agent to explore and update its policy in an given environment. To optimize agent interactions for task-specific learning with our universal buffer and pipeline, we introduce diverse communication patterns tailored for both single-agent and multi-agent environments. We evaluate the efficacy of our LTC approach on four diverse datasets: ALFWorld (single-agent), HotpotQA (multi-agent collaboration), Chameleon (multi-agent competition), and GSM8k (multi-agent teacher-student). On these data sets, LTC outperforms the supervised instruction fine-tuning baselines by 3.6% to 12%. These results highlight the versatility and efficiency of LTC in facilitating online adaptation for LLM agents.

==> curves_lm_loss.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.4]{figures/curves_alfworld_lm_loss.png}
  \caption{The loss curves of PPO training.}
  \label{fig:curves_lm_loss}
\end{figure}

==> curves_ppo_dev.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.4]{figures/curves_alfworld_dev.png}
  \caption{The acc curves for different generating sizes of each iteration.}
  \label{fig:curves_ppo_dev}
\end{figure}

==> curves_ppo_interaction.tex <==
% \begin{figure}[h]
%   \centering
%   \includegraphics[scale=0.4]{figures/curves_alfworld_ppo.png}
%   \caption{The acc curves of PPO training.}
%   \label{fig:curves_ppo}
% \end{figure}


% \begin{table}[t]
% \begin{wraptable}{br}{0.55\textwidth}
\begin{figure}[ht]
% \vspace{-10pt}
\centering
\small

    \centering
    % \includegraphics[scale=0.42]{figures/curves_alfworld_ppo.png}
    \includegraphics[scale=0.4]{figures/curves_alfworld_ppo.pdf}
    % \vspace{-10pt}
    \caption{The accuracy curves of PPO training.}
    \label{fig:curves_ppo}
    

% \vspace{-10pt}

\end{figure}


==> curves_ppo_loss.tex <==
% \begin{figure}[h]
%   \centering
%   \includegraphics[scale=0.4]{figures/curves_alfworld_ppo_loss.png}
%   \caption{The loss curves of PPO training.}
%   \label{fig:curves_ppo_loss}
% \end{figure}


% \begin{table}[t]
% \begin{wraptable}{br}{0.55\textwidth}
\begin{figure}[ht]
% \vspace{-10pt}
\centering
\small

    \centering
    % \includegraphics[scale=0.42]{figures/curves_alfworld_ppo_loss.png}
    \includegraphics[scale=0.4]{figures/curves_alfworld_ppo_loss.pdf}
    % \vspace{-10pt}
    \caption{The loss curves of PPO training.}

    \label{fig:curves_ppo_loss}
\vspace{-20pt}
\end{figure}


==> curves_ppo_train.tex <==
% \begin{figure}[h]
%   \centering
%   \includegraphics[scale=0.4]{figures/curves_alfworld_ppo.png}
%   \caption{The acc curves of PPO training.}
%   \label{fig:curves_ppo}
% \end{figure}


% \begin{table}[t]
% \begin{wraptable}{br}{0.55\textwidth}
\begin{figure}[ht]
\vspace{-10pt}
\centering
\small

    \centering
    % \includegraphics[scale=0.42]{figures/curves_alfworld_ppo_loss.png}
    \includegraphics[scale=0.42]{figures/curves_alfworld_ppo_loss.pdf}
    \caption{The loss curves of PPO training.}
    \label{fig:curves_ppo_loss}
% \vspace{-10pt}
\end{figure*}


==> curves_vs_if.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.4]{figures/curves_vs_if.png}
  \caption{The learning curves against instruction finetuning. \kuan{Put these curves to appendix}}
  \label{fig:curves_vs_if}
\end{figure}

==> fig_shortcut.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.38]{figures/shortcut.png}
  \caption{GPT-4 use some short-cuts to solve the problem.}
  \label{fig:shortcut}
\end{figure}

==> pipeline.tex <==
\begin{wraptable}{br}{0.5\textwidth}
% \begin{table}[ht]
% \vspace{-10pt}
\centering
\small

% \begin{figure}[h!]
  \centering
  \includegraphics[scale=0.3]{figures/pipeline.png}
  \caption{Illusion of the iterative training Pipeline. \kuan{this fig is just a placeholder}}
  \label{fig:overview}
% \end{figure}


% \vspace{-8pt}
\end{wraptable}

==> shortcuts.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.48]{figures/shortcuts.png}
  \caption{GPT-4 use some short-cuts to solve the problem. \kuan{put it into appendix}}
  \label{fig:shortcuts}
\end{figure}

==> table_gsm8k.tex <==
% \begin{table}[t]
\begin{wraptable}{br}{0.42\textwidth}
% \begin{table}[ht]
\vspace{-10pt}
\centering
\small
\begin{minipage}{.99\linewidth}
    \centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{llc}
\toprule
    %  \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method\footnote{\tiny HotpotQA EM is 27.1, 28.9, 33.8 for Standard, CoT, CoT-SC in \cite{wang2022rationale}.}}} & \textbf{HotpotQA}   \\
    % & (EM) \\ 
    \textbf{Model} & \textbf{Method} & \textbf{Accuracy}   \\
    \midrule
    % \multirow{4}{*}{PaLM-540B} & Standard  & 28.7 \\
    \multirow{2}{*}{PaLM-540B} & CoT{\scriptsize~\citep{wei2022chain}} & 56.5 \\ 
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 74.4\\
    % \midrule
    % &  Act  & 25.7 \\ 
 
    \midrule
    \multirow{2}{*}{GPT3-175B} & CoT{\scriptsize~\citep{wei2022chain}}   & 60.1 \\
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 78.0\\
    % & CoT-SC  $\to$ ReAct   & 34.2 \\
    % & ReAct $\to$ CoT-SC & \textbf{35.1}  \\ \midrule \midrule
    % & \textbf{Supervised SoTA\footnote{\tiny\citep{zhu2021adaptive,lewis2020retrieval}}} & 67.5 \\
    \midrule 
    \multirow{2}{*}{LLaMA-7B} & CoT{\scriptsize~\citep{touvron2023llama}} & 11.0 \\
    & CoT-SC{\scriptsize~\citep{touvron2023llama}}    & 18.1 \\
    \midrule \midrule
    \multirow{2}{*}{LLaMA-7B} & CoT-Tuning   & 37.7 \\
    & LTC   & \textbf{41.3} \\

    
\bottomrule
\end{tabular}%
}
\caption{
Accuracy on GSM8k. The results of the bottom block are obtained by fine-tuning LLaMA-7B model, while the others are prompting methods without fine-tuning. 
}
\label{tab:gsm8k}


\end{minipage}%

% \end{table}
\end{wraptable}

==> table_hotpotqa.tex <==
% \begin{table}[t]
\begin{wraptable}{br}{0.48\textwidth}
% \begin{table}[ht]
% \vspace{-10pt}
\centering
% \small
\begin{minipage}{.99\linewidth}
    \centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{llc}
\toprule
    %  \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method\footnote{\tiny HotpotQA EM is 27.1, 28.9, 33.8 for Standard, CoT, CoT-SC in \cite{wang2022rationale}.}}} & \textbf{HotpotQA}   \\
    % & (EM) \\ 
    \textbf{Model} & \textbf{Method} & \textbf{EM score}   \\
    \midrule
    % \multirow{4}{*}{PaLM-540B} & Standard  & 28.7 \\
    \multirow{3}{*}{PaLM-540B} & CoT{\scriptsize~\citep{wei2022chain}} & 29.4 \\ 
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 33.4\\
    % \midrule
    % &  Act  & 25.7 \\ 
    & ReAct{\scriptsize~\citep{yao2023react}}   & 27.4  \\
    & ReAct $\to$ CoT-SC & 35.1 \\
    \midrule
    GPT3-175B & ReAct   & 30.8 \\
    % & CoT-SC  $\to$ ReAct   & 34.2 \\
    % & ReAct $\to$ CoT-SC & \textbf{35.1}  \\ \midrule \midrule
    % & \textbf{Supervised SoTA\footnote{\tiny\citep{zhu2021adaptive,lewis2020retrieval}}} & 67.5 \\
    \midrule \midrule
    \multirow{2}{*}{PaLM-62B} & ReAct-Tuning   & 32.6 \\
    & CoT-Tuning   & 25.2 \\
    \midrule
    \multirow{2}{*}{PaLM-8B} & ReAct-Tuning   & 25.0 \\
    & CoT-Tuning   & 14.1 \\
    \midrule
    \multirow{2}{*}{LLaMA-7B} & ReAct-Tuning   & 28.1 \\
    & LTC   & \textbf{33.2} \\

    
\bottomrule
\end{tabular}%
}
\caption{
EM scores on HotpotQA with prompt and tuning methods. Methods that use fine-tuning are denoting with Tuning.
%The results of the bottom blocks are obtained by fine-tuning, while the others are prompting methods without fine-tuning from Table 1\&5 of~\cite{yao2023react}. PaLM-8b and PaLM-62B scores are estimates from Figure 3 of~\cite{yao2023react}.
% Prompting method results without fine-tuning are from Table 1\&5 of~\cite{yao2023react}. PaLM-8b and PaLM-62B scores are estimates from Figure 3 of~\cite{yao2023react}.
}
\label{tab:hotpotqa}


\end{minipage}%
% \hspace{5pt}
% \begin{minipage}{.57\linewidth}
%     \centering
    
%     \includegraphics[width=.49\textwidth]{iclr2023/figure/cots_scale.pdf}
%     \includegraphics[width=.49\textwidth]{iclr2023/figure/fever_cots_scale.pdf}
%     \captionof{figure}{PaLM-540B prompting results with respect to number of \reasons{} samples used.}
%     \label{fig:cots_to_react}
    
    


% \end{minipage}%
\vspace{-10pt}
% \end{table}
\end{wraptable}


==> table_hotpotqa_gsm8k.tex <==
% \begin{table}[t]
% \begin{wraptable}{br}{0.48\textwidth}
\begin{table*}[ht]
% \vspace{10pt}
\centering
% \small
\begin{minipage}{.38\linewidth}
    % \centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{llc}
\toprule
    %  \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method\footnote{\tiny HotpotQA EM is 27.1, 28.9, 33.8 for Standard, CoT, CoT-SC in \cite{wang2022rationale}.}}} & \textbf{HotpotQA}   \\
    % & (EM) \\ 
    \textbf{Model} & \textbf{Method} & \textbf{EM score}   \\
    \midrule
    % \multirow{4}{*}{PaLM-540B} & Standard  & 28.7 \\
    \multirow{3}{*}{PaLM-540B} & CoT{\scriptsize~\citep{wei2022chain}} & 29.4 \\ 
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 33.4\\
    % \midrule
    % &  Act  & 25.7 \\ 
    & ReAct{\scriptsize~\citep{yao2023react}}   & 27.4  \\
    & ReAct $\to$ CoT-SC & 35.1 \\
    \midrule
    GPT3-175B & ReAct   & 30.8 \\
    % & CoT-SC  $\to$ ReAct   & 34.2 \\
    % & ReAct $\to$ CoT-SC & \textbf{35.1}  \\ \midrule \midrule
    % & \textbf{Supervised SoTA\footnote{\tiny\citep{zhu2021adaptive,lewis2020retrieval}}} & 67.5 \\
    \midrule \midrule
    \multirow{2}{*}{PaLM-62B} & ReAct-Tuning   & 32.6 \\
    & CoT-Tuning   & 25.2 \\
    \midrule
    \multirow{2}{*}{PaLM-8B} & ReAct-Tuning   & 25.0 \\
    & CoT-Tuning   & 14.0 \\
    \midrule
    \multirow{2}{*}{Llama-7B} & ReAct-Tuning   & 28.2 \\
    & \modelshort {\tiny(single-agent monologue)}   & 31.0 \\
    & \modelshort {\tiny(multi-agent dialogue)}    & \textbf{33.2} \\
    \midrule
    \multirow{2}{*}{Llama2-13B} & ReAct-Tuning   & 33.8 \\
    & \modelshort {\tiny(multi-agent dialogue)}   & \textbf{35.8} \\


    
\bottomrule
\end{tabular}%
}
\caption{
EM scores on HotpotQA with prompt and tuning methods. Methods that use fine-tuning are marked by ``-Tuning''.
%The results of the bottom blocks are obtained by fine-tuning, while the others are prompting methods without fine-tuning from Table 1\&5 of~\cite{yao2023react}. PaLM-8b and PaLM-62B scores are estimates from Figure 3 of~\cite{yao2023react}.
% Prompting method results without fine-tuning are from Table 1\&5 of~\cite{yao2023react}. PaLM-8b and PaLM-62B scores are estimates from Figure 3 of~\cite{yao2023react}.
}
\label{tab:hotpotqa}


\end{minipage}%
\hspace{15pt}
\begin{minipage}{.44\linewidth}
    \centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{llc}
\toprule
    %  \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method\footnote{\tiny HotpotQA EM is 27.1, 28.9, 33.8 for Standard, CoT, CoT-SC in \cite{wang2022rationale}.}}} & \textbf{HotpotQA}   \\
    % & (EM) \\ 
    \textbf{Model} & \textbf{Method} & \textbf{Accuracy}   \\
    \midrule
    % \multirow{4}{*}{PaLM-540B} & Standard  & 28.7 \\
    \multirow{2}{*}{PaLM-540B} & CoT{\scriptsize~\citep{wei2022chain}} & 56.5 \\ 
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 74.4\\
    % \midrule
    % &  Act  & 25.7 \\ 
 
    \midrule
    \multirow{2}{*}{GPT3-175B} & CoT{\scriptsize~\citep{wei2022chain}}   & 60.1 \\
    & CoT-SC{\scriptsize~\citep{wang2022self-consistency}} & 78.0\\
    % & CoT-SC  $\to$ ReAct   & 34.2 \\
    % & ReAct $\to$ CoT-SC & \textbf{35.1}  \\ \midrule \midrule
    % & \textbf{Supervised SoTA\footnote{\tiny\citep{zhu2021adaptive,lewis2020retrieval}}} & 67.5 \\
    \midrule 
    \multirow{2}{*}{Llama-7B} & CoT{\scriptsize~\citep{touvron2023llama}} & 11.0 \\
    & CoT-SC{\scriptsize~\citep{touvron2023llama}}    & 18.1 \\
    \midrule \midrule
    \multirow{3}{*}{Llama-7B} & CoT-Tuning   & 37.7 \\
    & \modelshort {\tiny(single-agent monologue)}   & 39.6 \\
    & \modelshort {\tiny(teacher-student dialogue)}   & \textbf{41.3} \\

    
\bottomrule
\end{tabular}%
}
\caption{
Accuracy on GSM8k. The results of the bottom block are obtained by fine-tuning LLaMA-7B model, while the others are prompting methods without fine-tuning. 
}
\label{tab:gsm8k}


\end{minipage}%

% \vspace{-10pt}
\end{table*}
% \end{wraptable}


==> table_main.tex <==

\begin{table}[ht]
\centering
\begin{tabular}{l|ccc}
\textbf{Method / Dataset} & \textbf{GSM8k} & \textbf{Hotpot-QA} & \textbf{Alfworld} \\ 
\hline
\textbf{PaLM-540B + CoT/ReAct} & 46.9$^a$ & 29.4$^c$ & 70.9$^e$ \\ 
\textbf{GPT3-175B + CoT/ReAct} & 56.9$^b$ & 30.8$^d$ & 78.4$^f$ \\ 
\hdashline
\textbf{LLaMA-7B + Instruction Finetuning} & 37.7 & 28.1 & 64.2 \\ 
\textbf{LLaMA-7B + LTC} & \textbf{41.0} & \textbf{33.2} & \textbf{88.1}  \\
% \textbf{LLaMA + GPT4 Communication} & \textbf{41.0}\% & 30.1\% & -\%  \\
% \textbf{LLaMA + Self-feedback} & -\% & 30.1\% & -\%  \\
\end{tabular}
\caption{Iteractive feedback is better than instruction finetuning on three datasets. All metrics are accuracy (\%). Prior best numbers are from the following. a\&b:\cite{wei2022chain}. c\&d\&e\&f:\cite{yao2023react} \kuan{split it into 3 small tables and add more baselines}}
\label{tab:main}
\end{table}

==> table_patterns.tex <==


\begin{table}[h]
\centering
\begin{tabular}{l|ccc}
\textbf{Method / Dataset} & \textbf{GSM8k} & \textbf{Hotpot-QA} & \textbf{Alfworld} \\ 
\hline
\textbf{No Communication} & 37.7\% & 28.1\% & -\% \\ 
\textbf{Simple Reward PPO} & -\% & 33.2\% & -\%  \\
\textbf{GPT4 New Examples} & 41.0\% & -\% & -\%  \\
\textbf{Self-feedback} & -\% & 29.7\% & -\%  \\
\end{tabular}
\caption{Accuracy of different communication patterns on datasets}
\label{tab:my_label}
\end{table}
